Towards Automated Video Game Testing: Still a Long Way to Go

As the complexity and scope of game development increase, playtesting remains an essential activity to ensure the quality of video games. Yet, the manual, ad-hoc nature of playtesting gives space to improvements in the process. In this study, we investigate gaps between academic solutions in the literature for automated video game testing and the needs of video game developers in the industry. We performed a literature review on video game automated testing and applied an online survey with video game developers. The literature results show a rise in research topics related to automated video game testing. The survey results show that game developers are skeptical about using automated agents to test games. We conclude that there is a need for new testing approaches that did not disrupt the developer workflow. As for the researchers, the focus should be on the testing goal and testing oracle.

==> survey.tex <==

% lit -> survey -> conclusion
 
% To answer this question we
% (1) investigated X the academic literature to prepare interview questions;
% (2) interviewed X video game testers about its job and refined the questions;
% (3) surveyed the game tester community using the feedback from the interviewees; and
% (4) summarized and discuss the results.

% Our goal in this paper is
% (1) to understand how playtesting is done by interviewing professional playtesters; 
% (2) provide a formalisation (boxes and arrows, inputs, bpmn, uml...) of what is being done; and
% (3) discuss/propose/suggest what can be automated in this process.

\section{Method} \label{sec:method}

Playtesting and automated video game testing from the point of view of game testers

Testers opinions on automated game testing using AI

autom. game test (literature) -> survey questions -> conclusion

\subsection{Survey Objective}

% Each objective is simply a statement of the survey’s expected outcomes or a question that the survey is intended to answer.

The hypotheses to be tested
What alterative explanations are to be investigated or excluded
What scope of survey project is appropriate to address the objectives
What resources are necessary to achieve the objectives

\subsection{Survey Motivation}

What the purpose of the study is.
● Why it should be of relevance to them.
● Why each individual’s participation is important.
● How and why each participant was chosen.
● How confidentiality will be preserved.

The questionnaire is designed to discover what aspects of your educational background
have been useful to you in your career. The results of the survey will be used to help
improve curricula. All the information you provide will be kept confidential. In particular
we have no intention of judging you as a person–we are merely interested in learning about
the relevance of certain topics to your work.

\subsection{Survey documentation}

The objective(s) of the study.
A description the rationale for each question.
The rationale for any questions adopted or adapted from other sources, with appropriate citations.
A description of the evaluation process.

\subsection{}

Who the respondents were.
● How it was administered.
● How the follow-up procedure was conducted.
● How completed questionnaires were processed.

\subsection{Questions}

Divide the survey in two parts:
(1) First: general questions about the playtesting in general
(2) Second: specific questions about the last project the tester worked

Accessing playtesting: Outsourcing and freelance services (paid); social media specialized in game development like forums, Reddit, Linkedin, and Facebook.

\subsection{Sources}

\begin{itemize}
    \item VideoGame Professionals - Linkedin
    \item Software tester group - Linkedin
    \item Software Testing (QA) \url{https://www.facebook.com/groups/319410711488962/}
    \item Game Developers - \url{https://www.facebook.com/groups/gamedev}
    \item gamedev - \url{https://www.reddit.com/r/gamedev/} and Discord
    \item qa - \url{https://www.reddit.com/r/QualityAssurance/}
    \item Playtesters - \url{https://www.reddit.com/r/playtesters/}
    \item Discord - IGDA
\end{itemize}

\subsection{Questions}
Must be: about the process of testing and its workflow. What is the objective of Testing?
 
\begin{itemize}
    \item Gender
    \item Experience
    \item Do you play games normally as hobby?
    \item Which platform you playtest?
    \item Which game you playtest?
    \item Which equipment you use?
    \item How long you playtest?
\end{itemize}

\begin{enumerate}
    \item Experience with software
    \item Coding skills
\end{enumerate}

\begin{enumerate}
\item Do you receive an goal/objective from the devs before playtesting? Or do you playtest the game according to your understanding? Please elaborate
\item Do you use any kind of threshold? Like: "The game must run at 60 frames", "The level must take at least 5 min to complete.", "The weapon X should make the level easier".
\item Do you test the complete game?
\item Answer according with your experience as playtester. Why did you playtest for (objectives)? (list options from the literature and gray literature)
\item How do you playtest? (the steps) - open question
\item Do you follow a process?
\item How do tester communicate with the development team? 
\item How do you report the findings?
\item How do you replicate a problem/situation?
\item How often you playtest?
\item Do you playtest the same game over and over?
\item How does playtesting works for indie studios and big AAA studios?
\item Does the type of game change the way the way you test? How?
\item What aspect do you assess in the game? (fun, bugs, balance, etc)
\item How do you stress the game to find bugs?
\item You test the same thing for any game?
\end{enumerate}

on automation:

\begin{enumerate}
    \item How is it related to the game engine? 
    \item 
\end{enumerate}


\section{Survey Results} \label{sec:results}

...

\section{Formalization} \label{sec:formalization}

Analysis of the results and summary of the findings

\section{Discussion} \label{sec:discussion}

Propose a methodology derived from the insights of the playtesters:

\begin{itemize}
    \item Playtesting is more like a role based testing in traditional sw
    \item The playtesting is much more complex than sw Testing
    \item The regular tesing techniques might be applied to playtesting but it is not enough
    \item Real consequences in sw (people dying)
    \item Game dev has more complexity but less consequences
\end{itemize}

